The black hole occupation fraction of local dwarf galaxies with AXIS

The fraction of local dwarf galaxies that hosts massive black holes is arguably the cleanest diagnostic of the dominant seed formation mechanism of today's supermassive black holes. A 5 per cent constraint on this quantity can be achieved with AXIS observations of 3300 galaxies across the mass spectrum through a combination of serendipitous extra-galactic fields plus a dedicated 1 Msec GO program.

==> Definitions/journalnames.tex <==
\DeclareOption{ArXiv}{ 	    \gdef\@journal{ArXiv}	\gdef\@journalshort{ArXiv}	\gdef\@journalfull{ArXiv}	\gdef\@doiabbr{ArXiv}	}

